On the Complexity of Realizing Facial Cycles

We study the following combinatorial problem. Given a planar graph $G=(V,E)$ and a set of simple cycles $\mathcal C$ in $G$, find a planar embedding $\mathcal E$ of $G$ such that the number of cycles in $\mathcal C$ that bound a face in $\mathcal E$ is maximized. We establish a tight border of tractability for this problem in biconnected planar graphs by giving conditions under which the problem is NP-hard and showing that relaxing any of these conditions makes the problem polynomial-time solvable. Moreover, we give a $2$-approximation algorithm for series-parallel graphs and a $(4+\varepsilon)$-approximation for biconnected planar graphs.

==> makefile <==
finalname = maxfaces

psfiles = \


pdf:
	pdflatex $(finalname).tex



startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.backup

bib: 
	pdflatex $(finalname).tex
	bibtex $(finalname)
	pdflatex $(finalname).tex
	pdflatex $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o



print: ps
	lpr -Ppolaris -h $(finalname).ps

